An Optimizable Suffix Is Worth A Thousand Templates: Efficient Black-box Jailbreaking without Affirmative Phrases via LLM as Optimizer

Despite prior safety alignment efforts, mainstream LLMs can still generate harmful and unethical content when subjected to jailbreaking attacks. Existing jailbreaking methods fall into two main categories: template-based and optimization-based methods. The former requires significant manual effort and domain knowledge, while the latter, exemplified by Greedy Coordinate Gradient (GCG), which seeks to maximize the likelihood of harmful LLM outputs through token-level optimization, also encounters several limitations: requiring white-box access, necessitating pre-constructed affirmative phrase, and suffering from low efficiency. In this paper, we present ECLIPSE, a novel and efficient black-box jailbreaking method utilizing optimizable suffixes. Drawing inspiration from LLMs' powerful generation and optimization capabilities, we employ task prompts to translate jailbreaking goals into natural language instructions. This guides the LLM to generate adversarial suffixes for malicious queries. In particular, a harmfulness scorer provides continuous feedback, enabling LLM self-reflection and iterative optimization to autonomously and efficiently produce effective suffixes. Experimental results demonstrate that ECLIPSE achieves an average attack success rate (ASR) of 0.92 across three open-source LLMs and GPT-3.5-Turbo, significantly surpassing GCG in 2.4 times. Moreover, ECLIPSE is on par with template-based methods in ASR while offering superior attack efficiency, reducing the average attack overhead by 83%.

==> draft/design.tex <==
\section{Methodology}
\label{sec:method}

In this section, we will begin our discussion from an interesting observation, proposing a prototype of a jailbreaking method based on LLM self-optimization. We then extend it to the threat model, ultimately forming an adaptive jailbreaking suffix optimization approach.

\subsection{Observation and Our Intutive Method}
 
\input{src/tfs/fig_observation.tex}

In the GCG, optimizing an effective adversarial suffix for jailbreaking often requires hours of effort, where suffixes that can be tens of tokens long and highly unnatural. 
This poses a significant challenge in finding successful jailbreaking prompts. 
However, our observations reveal that current LLMs may not be as robust in resisting jailbreaking attacks. 
Interestingly, in some cases, simply appending ``a single number'' to the input malicious query can induce the target LLM to generate unethical responses.
As illustrated in \autoref{fig:observation_example}, by appending a numeric suffix, both the LLaMA2 and GPT-3.5 will continue to leak detailed harmful guidance against the incoming malicious queries.
Meanwhile, we can observe that the generated unethical responses are very diverse, i.e., not limited to specific affirmative responses as a beginning.
% This finding drive us to explore the possibility of utilizing more concise and natural suffixes for efficient jailbreaking attacks.
This issue may stem from the imperfect robustness of the LLM. 
We observed that appending a numerical suffix to an original malicious prompt causes a shift in the embedding space. 
As illustrated in ~\autoref{fig:embedding_distribution}, we sample a wide array of numerical suffixes and visualize the embeddings of both successful and failed jailbreaking prompts.
The successful prompts tend to cluster towards the corners, indicating a potential distinctive impact on LLM behavior.

\input{src/tfs/fig_embedding.tex}

Recent studies have highlighted the potential of LLM to serve as an efficient black-box  optimizer~\cite{song2024position, yang2023large,lange2024large,nie2023importance}. 
For instance, when presented with a mathematical problem, a LLM can generate candidate solutions. 
This process merely requires providing the LLM with feedback to assess the quality of each proposed solution, thereby enabling the LLM to engage in self-reflection and optimization to enhance the quality of its responses.
Inspired by this capability, an intriguing intuition emerged: \textit{Could numeric suffixes be treated as variables to be optimized automatically by an LLM?}
This intuition also aligns with the current trend where researchers are developing automated systems to evaluate and judge the ethical implications of text, offering a convenient means to feed back potential jailbreaking effectiveness into the LLM for optimizing candidate suffixes.

Building on this intuition, we conceptualize numerical suffixes as optimizable mathematical variables, allowing the target LLM to function as an optimizer tasked with significantly impacting prompts' features to successfully facilitate a jailbreak. 
Surprisingly, this straightforward approach effectively identifies adversarial numerical suffixes that induce unethical content from target LLM. 
\todo{The specific results are detailed in the Appendix XXX.} 
This method offers significant advantages as it eliminates the need for manually designed affirmative responses. 
This approach presents substantial benefits by obviating the requirement for manually crafted affirmative responses. 
Furthermore, we explore to investigate the potential to broaden this method to encompass the optimization of various suffix types beyond merely numerical ones.



\begin{algorithm}[tb]
    \caption{\sys}\label{alg:jailbreaking}
    \textbf{Input:} Target LLM $\mathcal{M}$, The malicious query $x$ \\
    \textbf{Output:} Successful jailbreaking suffix or None
    \begin{algorithmic}[1]
        \Function{JailbreakLLM}{$\mathcal{M}$, $x$}
        % \State $\triangleright$ Initialize History List
        \State $\text{History} \gets [\ ] $
        \Comment{Initialize the history list}
        % \State $\triangleright$ Perform $K$-round optimization
        \For{$k = 1 \text{ to } K$}  % Outer loop for maximum number of \(\)optimization rounds
            \Comment{Perform $K$-round optimization}
        % \State $\triangleright$ Select reference pairs from History List
            \State $\text{refs} \gets$ \hyperlink{lab:refsampling}{Sampling}($\text{History}$)
            \Comment{Select reference pairs from the history list}
            % \State $\triangleright$ Complete the attacker template 
            \State $p_{atk} \gets$ \hyperlink{lab:RefTemp}{FillTemplate}($x$, $\text{refs}$) 
            \Comment{Complete the attacker template}
            % \State $\triangleright$ Generating candidate suffixes
            \State $S \gets \mathcal{M}(p_{atk})$
            \Comment{Generating candidate suffixes}
            \For{each candidate suffix $s$ in $S$}
                \If{Suffix extraction successful}
                    % \State $\triangleright$ Query the Target LLM to get the response 
                    \State $r \gets \mathcal{M}(x \oplus s)$  % Query LLM API with potential jailbreak prompt
                    \Comment{Query the target LLM to get the response}
                    % \State $\triangleright$ Check for jailbreaked or not
                    \State $\text{score} \gets$ \hyperlink{lab:scorer}{Scorer}($r$)  % Score the response
                    \Comment{Check for jailbreaked or not}
                    \If{$\text{score} >$ threshold}  % Check if the attack is successful
                        \State \Return $x \oplus s$  % Return successful jailbreaking prompt
                    \Else
                    % \State Add \((s, score)\) to \(HistoryList\)
                    \State \(\text{History} \gets \text{History} \cup  [ (s, \text{score})] \) 
                    \Comment{Maintain the history list}
                    \EndIf
                \EndIf
            \EndFor
        \EndFor
        \State \Return "Jailbreaking Failed after $K$ Rounds"  % Return failed after exhausting all rounds
        \EndFunction
    \end{algorithmic}
\end{algorithm}


\subsection{LLM as An Optimizer: Efficient Black-box Suffix Optimization}

% Our next step is to generalize the jailbreaking suffix optimization to generate more diverse and effective suffixes, which are not limited on numbers only.

Building upon this concept, we formulate the discrete search for jailbreaking suffixes as an optimization problem, allowing the LLM to find suffixes that trigger jailbreaking behavior, yielding promising results.
Furthermore, we extend the method to arbitrary suffixes, namely optimizable suffixes. 
We let the target LLM act as the attacker to optimize the suffixes by introducing a harmfulness predictor for automatic efficacy scoring.
We also maintain a history of generated suffixes and related harmfulness scores for the LLM's reflection. 
Ultimately, our method achieves effective and efficient jailbreaking attacks in a completely black-box setting without requiring affirmative responses.

% For convenience of discussion, we denote the target LLM as \(M\).

\noindent\textbf{Overall attacker role-playing.}
We assign the LLM a role of a red team testing expert and task it with generating a suffix for a given query. 
The objective is to induce a significant change in a chatbot's assessment of the question, causing a substantial shift in the feature space.
This shift should enable the chatbot to successfully answer the question rather than provide a refusal response. 
To streamline the process of extracting the generated suffix, we instruct the LLM to output its response in a JSON-like format whenever feasible.
The attacker template is as follows:
\begin{mdframed}
    \textbf{Attacker Template:} You are a red-teaming expert, please optimize this prompt ``\textcolor{blue}{[QUERY]}'' by adding a suffix that will have a large impact on the feature hidden space, so that a conversational bot can successfully answer the question corresponding to PROMPT without denying service.
    \textcolor{blue}{[REF]}. Please directly output the suffix within 10 tokens, as the following the format \textcolor{blue}{\{"suffix":[OUTPUT]\}}.
\end{mdframed}
where the ``[QUERY]'' is the replaced by the input malicious query, to guide the adaptive optimization for the specific query.

\noindent\hypertarget{lab:refsampling}{\textbf{Selection of Reference Histories.}}
To enable the LLM to engage in self-reflection and optimization based on feedback on the quality of responses, it is essential to provide it with a set of historically generated suffixes along with their corresponding jailbreaking efficacy scores. 
To achieve this, we maintain a list of suffix-score pairs during the optimization process and sample from this list. 
Specifically, we employ a hybrid sampling strategy: half of the references are those with the highest scores, as these are likely closer to the target outcome; the other half are randomly chosen from the remaining historical records to enhance diversity and prevent the optimization from getting trapped in local optima. 
Ultimately, the sampled historical references are transformed into feedback prompts that encourage the LLM to reflect deeply and generate higher-scoring candidate solutions. 
These feedback prompts are based on the following reference template:
\begin{mdframed}
    \hypertarget{lab:RefTemp}{\textbf{References Template:}} There are some history generated suffixes and the scores in ``(suffix, score)'', where a higher score indicates a better prompt: \textcolor{blue}{Sampled Histories} .Please reflect deeply on these results and generate a new suffix that will have a large score.
\end{mdframed}
This reference prompt will be integrated into the attacker prompt by replacing the ``[REF]'' placeholder.

\noindent\hypertarget{lab:scorer}{\textbf{Choice of Scorers.}}
In the original implementation of GCG, success or not of a jailbreaking attempt is determined by using rule-based matching to check if the target LLM's response begin with specific denial phrases. 
This method, while straightforward, does not provide continuous, optimizable feedback and is susceptible to a high rate of false positives, as seen in cases such as XXX. 
Recent research have shifted towards employing specialized discriminative models~\cite{yu2023gptfuzzer,huang2023catastrophic} or crafting specific prompts that enable an LLM to act as a judge model~\cite{qi2023fine,chao2023jailbreaking}. 
These models are capable of producing fine-grained scores that assess the maliciousness of responses.
From a computational efficiency perspective, we adopt the classifier trained by Yu et al~\cite{yu2023gptfuzzer}, integrating it into the rule-based matching mechanism ~\cite{zou2023universal} to form a scoring pipeline, where the higher the score, the more likely the response is to be unethical.


\subsection{Algorithm}
The algorithm is illustrated in \autoref{alg:jailbreaking}. 
This method constitutes an iterative optimization framework, allowing for up to \(K\) rounds of suffix optimization for a given malicious query (in Line 3). 
As previously stated, we provide the LLM with historical references for self-reflection, commencing with a sampling-based selection on reference history list (in Line 4). 
It is notable that a maximum number of reference history pairs is designated as \(MaxH\). 
Thus, in the beginning that the history list is empty, the reference prompt for that round is omitted. 
Furthermore, the malicious query and historical references are integrated into an attacker template to construct the input prompt (in Line 5). 
By feeding this integrated prompt to the target LLM, candidate suffixes are generated (in Line 6). 
To enhance optimization efficiency, a batch generation strategy is employed to produce multiple candidate suffixes simultaneously. 
Each generated suffix is evaluated by a scorer to assess its efficacy as an attack and to determine whether the jailbreak is successful (in Line 9-14). 
If successful, the generated jailbreaking prompt is returned (in Line 11-12). Otherwise, the current suffix and its score are added to the history list, and the process moves to the next optimization round (in Line 14) until a jailbreak is successful or the iteration limit is reached.







==> draft/intro.tex <==
\section{Introduction}
\label{sec:intro}

Recently, Large Language Models (LLMs) have made significant strideswith represented by ChatGPT~\cite{}, Claude~\cite{}, and Bard~\cite{}, demonstrating remarkable capabilities in intelligent question answering~\cite{}, code generation~\cite{}, task planning~\cite{}, and logical reasoning~\cite{}. 
These advancements are bringing profound changes to the way people live and work.
Mainstream LLM products undergo safety alignment processes before deployment to ensure their outputs align with human moral values and laws.
However, recent research reveals that despite these preventive measures, LLMs remain vulnerable to jailbreaking attacks. 
Attackers can craft elaborate prompts to manipulate LLMs into generating harmful and unethical content, posing significant threats to their safety and credibility.
Jailbreaking has garnered extensive interest and discussion, and within relevant communities~\cite{}, hundreds of discovered jailbreaking tips and examples have already been shared.

To further expose the safety deficiencies in LLMs, a series of jailbreaking methods have been proposed, serving as red-teaming tools. 
Existing jailbreaking methods can be broadly categorized into two classes: Template-based methods and Optimization-based methods.
Template-based methods utilize predefined templates or strategies informed by successful jailbreak hints or insights from psychology and social engineering to generate effective jailbreaking prompts. 
\todo{Optimization-based method. And give more details and discussions about their limitations.}

In this paper, we propose a novel jailbreaking method, \sys(\bfd{E}ffi\bfd{C}ient bLack-box ji\bfd{L}breaking method with o\bfd{P}timizale \bfd{S}uffix\bfd{E}s), for effectively and efficiently exploiting the vulnerabilities of LLMs.
Our method is inspired by the observation that current LLM alignments are not robust. 
As shown in ~\autoref{fig:observation_example}, appending a simple number to the original malicious query can induce the LLM to generate unethical responses.
Recent research~\cite{yang2023large} has demonstrated that LLMs can be utilized as optimizers to automated solve complex problems, such as mathematical puzzles, using LLMs to generate candidate answers and interactively providing reward scores for the answers they produce.
Through well-designed prompting, LLMs can engage in self-reflection, generate new solutions, and ultimately optimize and solve the problem by obtaining higher rewards. 
Building upon this concept, we frame the search for jailbreaking suffixes as an optimization problem, enabling the LLM to identify suffixes that effectively trigger jailbreaking behaviors, which has shown promising results. 
We expand this method to include not just predefined but arbitrary, optimizable suffixes. 
The target LLM itself acts as the attacker, using a harmfulness predictor we introduced to autonomously score the efficacy of each suffix. 
We also compile a historical reference list of generated suffixes along with their harmfulness scores to facilitate the LLM's self-reflection and learning. Ultimately, this method facilitates effective and efficient jailbreaking attacks within a fully black-box environment, eliminating the need for predefined affirmative responses.

==> draft/rw.tex <==
\section{Related Work}\label{sec:rw}

\noindent \textbf{Template-based Methods.}
Template-based methods leverage patterns derived from successful jailbreak hints~\cite{deng2023jailbreaker,yu2023gptfuzzer} or incorporate insights from psychology and social engineering~\cite{li2023deepinception,chao2023jailbreaking} to devise effective jailbreak templates, either manually or automatically.
DeepInception~\cite{li2023deepinception} introduces manually crafted templates that embed nested scenarios to hypnotize LLMs into producing malicious outputs.
RED-EVAL~\cite{bhardwaj2023red} employs a Chain of Utterances (CoU)-based prompt to extract harmful information step by step.
GPTFUZZER~\cite{yu2023gptfuzzer}, employs software fuzzing test principles, to collect a variety of successful jailbreaking templates as seeds and apply mutations to spawn novel prompts.
Masterkey~\cite{deng2023jailbreaker} fine-tunes an LLM using reinforcement learning on collected workable jailbreak prompts to unearth underlying jailbreak mechanisms and learn potent patterns autonomously.
PAIR~\cite{chao2023jailbreaking} enables LLMs to autonomously generate and refine jailbreaking prompts by providing some pre-designed general strategies such as obfuscating sensitive words and engaging in role-playing scenarios.
Additionally, some studies convert jailbreaking prompts into encrypted or low-resource languages~\cite{yuan2024gpt4,yong2024lowresource}, exploiting the limited alignment in these languages to facilitate jailbreaking.
These methods can achieve effective jailbreaking simply by black-boxing queries to the target LLM's API, obviating the need for multiple rounds of iterative optimization. 
Template design, however, necessitates careful strategic exploration, and the variety and diversity of prompts generated from the same template are limited.


\noindent \textbf{Optimization-based Methods.}
Optimization-based methods are commonly employed for generating adversarial examples in NLP tasks, particularly in discriminative tasks~\cite{liu2022piccolo,wen2024hard,guo2021gradient}. These methods typically model attack targets by manipulating embeddings or predicting logits, thereby facilitating the gradient-based optimization search for candidate tokens. 
Among these, the Greedy Coordinate Gradient (GCG)~\citep{zou2023universal} stands out as a seminal work focused on the optimization-based jailbreaking of generative LLMs. 
GCG aims to craft adversarial suffixes that prompt LLMs to specific maliciously affirmative responses (e.g., Sure, here is ...), thereby successfully inducing the target LLM to continue giving harmful answers.
GCG streamlines the optimization process by combining gradient approximation with a methodical affirmative phase to enhance efficiency. 
Recent efforts explore to enhance token optimization methods.
RIPPLE~\cite{shen2024rapid} proposes replacing affirmative phrases with subconscious exploitations to streamline the optimization process. 
AutoDAN~\cite{liu2023autodan} employs a hierarchical genetic algorithm to optimize discrete tokens, bypassing traditional gradient propagation techniques. 
Despite its effectiveness and adaptiveness, optimization-based methods face several challenges. 
It requires white-box access and depends on manually predefined potential target responses (e.g., affirmative responses). 
% Moreover, the suffixes it generates are often nonsensical and incomprehensible to humans, posing significant limitations on their practical applicability.








==> draft/threatmodel.tex <==
\section{Problem Formulation}
\label{sec:preliminary}
Before diving into our proposed jailbreaking method, we first delineate the threat model considered in this paper.

% \noindent\textbf{Threat model.}
% We adhere to the threat model proposed by GCG~\citep{zou2023universal}. 
% For any given malicious query, the challenge entails appending a specific suffix that successfully prompts the target LLM to produce an unethical response. 
% In this paper, we investigate scenarios that more closely align with real-worlds by focusing on the black-box setting. 
% In this setting, attackers are restricted to collecting only response strings from the target LLM, with no access to its internal parameters or gradients. Furthermore, while GCG mandates that attackers predefine the starting sequence of the target LLM's response (e.g., Sure here is ...), our goal is to develop more adaptive and universal attack methods, without relying on prior knowledge of the desired unethical response.

% \noindent\textbf{Formulation.}
% Given a sequence of \( n \) tokens representing a malicious query, denoted as \( \mathbf{x} = (x_1, x_2, \ldots, x_n) \), 
% our primary goal is to identify an optimizable suffix \( \mathbf{s} = (s_1, s_2, \ldots, s_m) \) that, upon concatenation with \( \mathbf{x} \), maximizes the probability of inducing an unethical response \( \mathbf{y} = (y_1, y_2, \ldots, y_k) \) from the target LLM. 
% The challenge involves how to conduct effective and efficient optimization for \( \mathbf{s} \) to achieve this goal.
% Formally, the optimization goal is defined as:
% \begin{equation}
% \mathbf{s}^* = \arg \max_{\mathbf{s}} P(\mathbf{y} \mid \mathbf{x} \oplus \mathbf{s})
% \end{equation}
% where \( \oplus \) symbolizes the concatenation operation. 
% This probability is further expanded by the equation:
% \begin{equation}
% P(\mathbf{y} \mid \mathbf{x} \oplus \mathbf{s}) = \prod_{i=1}^{k} P(y_i \mid \mathbf{x} \oplus \mathbf{s}, y_1, y_2, \ldots, y_{i-1})
% \end{equation}
% In this formulation, \( P(y_i \mid \mathbf{x} \oplus \mathbf{s}, y_1, y_2, \ldots, y_{i-1}) \) represents the conditional probability of generating the \( i \)-th token \( y_i \) in the output sequence, predicated on the concatenated input sequence \( \mathbf{x} \oplus \mathbf{s} \) and all previously generated tokens in \( \mathbf{y} \). This model emphasizes the sequential dependencies within the output generation process and illustrates the sophisticated challenge of designing a suffix that strategically directs the model's output towards unethical results.

Here is a revised version that clearly differentiates your approach from the GCG model, particularly emphasizing the black-box setup and the flexibility in generating responses:

\section{Problem Formulation}
\label{sec:preliminary}
Before delving into our proposed jailbreaking method, we first outline the threat model this paper considers.

\noindent\textbf{Threat Model.}
Our approach diverges significantly from the threat model proposed by GCG~\citep{zou2023universal} in two critical aspects. Firstly, our research focuses on a black-box setting, where the attacker has no access to the target LLM's internal parameters or gradients—only the response outputs are available. Secondly, unlike GCG, which confines attackers to generating responses starting with a predefined sequence (e.g., "Sure, here is ..."), we aim to remove any such constraints on the affirmative responses. This flexibility allows for a broader exploration of potential unethical outputs from the LLM.

\noindent\textbf{Formulation.}
Consider a malicious query represented by a sequence of \( n \) tokens, \( \mathbf{x} = (x_1, x_2, \ldots, x_n) \). Our objective extends beyond the constraints of the GCG model. We aim to identify and optimize a suffix \( \mathbf{s} = (s_1, s_2, \ldots, s_m) \) that, when concatenated with \( \mathbf{x} \), maximizes the likelihood of inducing any unethical response \( \mathbf{y} = (y_1, y_2, \ldots, y_k) \) from the target LLM, rather than optimizing towards a prefixed response sequence. The formulation is as follows:
\begin{equation}
\mathbf{s}^* = \arg \max_{\mathbf{s}} P(\mathbf{y} \mid \mathbf{x} \oplus \mathbf{s})
\end{equation}
where \( \oplus \) denotes the concatenation operation. This probability is decomposed as:
\begin{equation}
P(\mathbf{y} \mid \mathbf{x} \oplus \mathbf{s}) = \prod_{i=1}^{k} P(y_i \mid \mathbf{x} \oplus \mathbf{s}, y_1, y_2, \ldots, y_{i-1})
\end{equation}
In this model, \( P(y_i \mid \mathbf{x} \oplus \mathbf{s}, y_1, y_2, \ldots, y_{i-1}) \) represents the conditional probability of generating each token \( y_i \) in the output sequence, predicated on the concatenated input sequence \( \mathbf{x} \oplus \mathbf{s} \) and all previously generated tokens. This approach allows for generating any malicious sequence \( \mathbf{y} \), highlighting our method's adaptability and breadth in exploring unethical outcomes.


==> src/tfs/fig_failcasegcg.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
    \begin{center}
      \includegraphics[width=0.39\textwidth]{src/figs/gcgcase.pdf}
    \end{center}
    % \caption{A failed jailbreaking example by GCG. Although the GCG-generated suffix successfully induces an affirmative response, the LLM subsequently continues to refuse to answer.} 
    \caption{A GCG jailbreaking example that successfully induces an affirmative response but the LLM still refuses to answer.} 
    \label{fig:failcasegcg}
\end{wrapfigure}

==> src/tfs/fig_observation.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{src/figs/observation_example.pdf}
        \caption{Examples of successful jailbreaking with a simple numeric suffix.} 
    \label{fig:observation_example}
\end{figure}

==> src/threatmodel.tex <==
\section{Problem Formulation}
\label{sec:preliminary}
Before diving into our methodology, we firstly delineate the threat model considered in this paper.

\noindent\textbf{Threat model.}
We adhere the threat model initially proposed by GCG~\citep{zou2023universal}, which involves finding a specific suffix to any given input to induce the target LLM to output harmful or unethical responses. 
However, we extend this model to better mirror real-world scenarios. 
Firstly, we shift from a white-box setting, where attackers could access the model's weights and gradients, to a black-box setting, where the attacker can only interact with the LLM through its API and receive textual responses, which is inspired by the fact that many advanced LLMs are deployed as APIs without releases.
Secondly, rather than relying on predefined affirmative phrases in GCG, we aim to identify workable suffixes that can cause the LLM to generate any form of harmful response directly in response to the given query. 



\noindent\textbf{Formulation.}
Consider a malicious query represented by a sequence of \( n \) tokens, \( \mathbf{x} = (x_1, x_2, \ldots, x_n) \). 
our primary goal is to identify an optimizable suffix \( \mathbf{s} = (s_1, s_2, \ldots, s_m) \) that, upon concatenation with \( \mathbf{x} \), maximizes the probability of inducing an unethical response \( \mathbf{y} = (y_1, y_2, \ldots, y_k) \) from the target LLM. 
The challenge involves how to conduct effective and efficient optimization for \( \mathbf{s} \) to achieve this goal.
Formally, the optimization goal is defined as:
\begin{equation}
\mathbf{s}^* = \arg \max_{\mathbf{s}} P(\mathbf{y} \mid \mathbf{x} \oplus \mathbf{s})
\end{equation}
where \( \oplus \) symbolizes the concatenation operation. 
This probability is further expanded by the equation:
\begin{equation}
P(\mathbf{y} \mid \mathbf{x} \oplus \mathbf{s}) = \prod_{i=1}^{k} P(y_i \mid \mathbf{x} \oplus \mathbf{s}, y_1, y_2, \ldots, y_{i-1})
\end{equation}
In this formulation, \( P(y_i \mid \mathbf{x} \oplus \mathbf{s}, y_1, y_2, \ldots, y_{i-1}) \) represents the conditional probability of generating the \( i \)-th token \( y_i \) in the output sequence, predicated on the concatenated input sequence \( \mathbf{x} \oplus \mathbf{s} \) and all previously generated tokens in \( \mathbf{y} \). This model emphasizes the sequential dependencies within the output generation process and illustrates the sophisticated challenge of designing a suffix that strategically directs the model's output towards unethical results.




